Metric Learning for Adversarial Robustness

Deep networks are well-known to be fragile to adversarial attacks. We conduct an empirical analysis of deep representations under the state-of-the-art attack method called PGD, and find that the attack causes the internal representation to shift closer to the "false" class. Motivated by this observation, we propose to regularize the representation space under attack with metric learning to produce more robust classifiers. By carefully sampling examples for metric learning, our learned representation not only increases robustness, but also detects previously unseen adversarial samples. Quantitative experiments show improvement of robustness accuracy by up to 4% and detection efficiency by up to 6% according to Area Under Curve score over prior work. The code of our work is available at https://github.com/columbia/Metric_Learning_Adversarial_Robustness.

==> source/related_bck.tex <==
%auto-ignore
\section{Preliminary Knowledge and Related Work}
\label{sec:prelim}
\vspace{-1em}

This work is built upon the prior work on Adversarial Attacks and use of triplet-loss to representation learning. We briefly describe them below. Please refer to [\cite{corr/GoodfellowSS14}, \cite{BIM}, \cite{madry}, \cite{CW}, \cite{mim}, \cite{stability_training}, \cite{ALP}] for more details. We first introduce some notations that we will follow in the rest of the paper.

% \medskip   $F(\x,\tha)  
% Denote the set of activations in the $FC$ corresponds to the penultimate
% layer (since these correspond to inputs to a linear classifier) as $h(\x)$~\bray{check if this line fits somewhere else}.

% Specifically, denote $\mathcal{L}_{ce}(F(\x),y)$ to be the cross-entropy loss, which is usually used as the training objective for standard[] deep learning models. 

\noindent
\textbf{Notations.}
Let $M$ to be the number of classes to predict and $N$ to be the number of examples in the training set. We formulate the DNN classifier as $F(\x)\in \mathbb{R}^M$ to be a probability distribution, where $\x$ is the input variable. We denote $\mathcal{L}(F(\x), y)$ to be the standard loss function for image recognition. We also denote $\I(\x, \epsilon)$ to be the $l_\infty$ ball centered at $\x$ with radius $\epsilon$.

% Without loss of generality, we assume that the network we study has $n\geq 3$ layers, where the softmax layer is the $n$-th layer and the pre-softmax layer is the $(n-1)$-th layer. The representation of the $i$-th layer is denoted as $h_i(\x)$. 

 \subsection{Adversarial Attacks}
 We focus on robustness against $l_{\infty}$ bounded, untargeted adversarial attacks. The objective of the $l_{\infty}$ attacks is to generate $\x' \in \I(\x, \epsilon)$ such that $F(\x') \neq F(\x)$. We use the following attacks: 


\textbf{Fast Gradient Sign Method (FGSM)} [\cite{corr/GoodfellowSS14}] generates adversarial examples $\x'$ by $\x'=\x+\epsilon \cdot \textrm{sign}(\nabla_\x \mathcal{L}(F(\x),y))$ with a single step.

\textbf{Basic Iterative Method (BIM)} [\cite{BIM}] is a straightforward extension of FGSM by applying it multiple times with small steps, where the update formula at the i-th step is: $\x'_i = \textrm{clip}_{\x, \epsilon}(\x'_{i-1} + \alpha \cdot \textrm{sign}(\nabla_{\x'_{i-1}} \mathcal{L}(F(\x'_{i-1}), y)) )$, where $\alpha$ is the step size.


\textbf{Projected Gradient Descent (PGD)} [\cite{madry}] is a variant of the BIM method, where the starting point $\x_0$ is in $\I_\epsilon(\x)$. It can be made more powerful by randomly starting several times and calculating the union of the mispredictions.

\textbf{Carlini \& Wagner (C\&W)} [\cite{CW}] We reformulate the C\&W method to $l_{\infty}$ attack as in [\cite{madry}].
We generate $\x'$ by minimizing the loss $g(x):=\max_\x{(\max_i{\{z(\x)_i: i \neq t\}}-z(\x)_t, - \kappa)}$, where $z(\x)=\textrm{logit}(h_{n-1}(x))$ and $\kappa$ controls the confidence on adversarial examples.


\textbf{Momentum Iterative Method (MIM)} [\cite{mim}] is a BIM with momentum which won the NeurIPS 2017 Adversarial Competition. MIM updates the gradient $g_i = \textrm{momentum} \cdot g_{i-1} + \nabla_{\x'_{i-1}} \mathcal{L}(F(\x'_{i-1}), y)) $ with momentum at each iteration, and generates the attack iteratively with $\x'_i=\textrm{clip}_{\x, \epsilon}(\x'_{i-1}+\alpha \cdot \textrm{sign}(g_i))$.

\textbf{Black-box Attacks (BB)} [\cite{blackbox}] Black-box attack is to generate adversarial examples on one model and transfer them to the target models. In this paper, we generate the adversarial attacks with PGD on the substitute model and conduct black-box attack to the evaluated models.

% In this paper, we adopt the well studied PGD attack for black-box attacks .

% \textbf{SPSA} [\cite{pmlr-v80-uesato18a}] attack is based on the gradient-free optimization, which approximates the analytic gradients with finite difference estimates in random directions. It is effective under obfuscated gradients.


% Denote $q(\x):=-\mathcal{L}(F(\x), y)$ to be the function to minimize by the SPSA attack. At the t-th iteration, it calculates the approximate gradient $\g_i=(q(\x_t+\delta \v_i)-q(\x-\delta \v_i))\v_i^{-1}/(2 \delta)$, where $\delta$ is the perturbation size and $\v_i$ is sampled uniformly from $\{1, -1\}^D$, then set $\x'_t = \x_t - \alpha(1/n)\sum_{i=1}^{n}\g_i$, where $\alpha$ is the step size, and project back the perturbed example $\x_{t+1}=\argmin_{\x \in N_{\epilon}(\x_0)}||\x'_t-\x||$.



% generates adversarial example using the formula $\x'(\omega)=\frac{1}{2} (\tanh (\omega)+1)$, where $\omega = \argmin_\omega ||\x'(\omega)-\x||_2^2+c \cdot g(\x'(\omega))$, where $c$ is a constant found by a modified binary search and , . 



\subsection{Robust Training Methods}

% [do you think this is too isolated.]

%  A line of research has been conducted via the adversarial training method to defend neural networks against adversarial perturbations [\cite{intriguing}, \cite{madry}]. is shown to be powerful in regularizing and training robust DNNs [\cite{intriguing}].
 

 \textbf{Adversarial training (AT)} [\cite{madry}] achieves benchmark adversarial robustness by training the neural network on the created adversarial examples, which goes through densely scrutiny and its robustness is endorsed by Athalye et al [\cite{obfuscated}]. The formulation is proposed as the following: $\min_{\tha}{\rho(\tha)}, \textrm{where } \rho(\tha) = \mathbb{E}_{(\x,y) \sim \D }{[\max_{\delta \in S}\mathcal{L}(\tha, \x+\delta, y)]}$, where $S \in \I(\x, \epsilon)$.

% Our method innovatively modifies the triplet data by pulling the adversarial examples $a'$ and the negative examples $n$ apart to achieve a safe margin between those two. 

\textbf{Adversarial Logit Pairing (ALP)} [\cite{ALP}] builds on top of [\cite{madry}] and introduces an additional loss term that matches the logits from a clean image $\x$ and its corresponding adversarial image $\x$. However, this method has been known to have a distorted loss function and is not scalable to untargeted attack [\cite{evaluateALP}, \cite{LPfool}]. Contrary to this, our method learns to separate the adversarial embedding to the potential dangerous negative samples with margins.

%  proposes to train stable feature embeddings on natural transformations of original image. It

Several other robust training methods do not focus on the $L_{\infty}$ adversarial attack, so we do not compare them with our method in the experiment section.  In particular, stability training regularizes the natural loss with  $L_{stability}(\x,\x')=||h(\x)-h(\x')||_2$, where $\x'$ is the result of some natural transformation such as rotation, not adversarial attack. Stability training was demonstrated to improve the robustness of a metric learning based model, whereas our method leverages metric learning to improve the robustness of general networks.  DeepDefense [\cite{deepdefense}] considers an adversarial attack directly in the loss function without generating adversarial examples. Model ensemble is another way to improve robustness [\cite{ensemble}, \cite{PED}].

% , which matches the features of the original images ${a, p, n}$ with that of the naturally transformed images ${a',p', n'}$ respectively (This method focuses on natural transformation instead of adversarial perturbations). 

% improves the adversarial accuracy on top of Madry et al. 's method. It introduces some regularization to the logit feature layer by matching the logit of original images and the corresponding adversarial images.


% Siamese Network variants train the network to distinguish similar and difference paris of examples by encouraging images of one class to be projected onto a single point in the representation. On the other hand, the triplet loss tries to enforce a margin between different classes [\cite{facenet}].

% !Modify Triplet loss has made progress in embedding learning over the past decades. Usually, its input consists of three parts, an anchor $\x_i$, a positive example $\x^+_j$, and a negative example $\x^-_k$. 

% The anchor and the positive examples belong to the same class, and the negative sample belongs to a different class. Triplet loss can learn embeddings with a significant margin, as the margin nearest neighbor shown by Weinberger et al. [\cite{LMNN}], which pushes the anchor and the positive sample together and creates a large margin with the negative example. The selection of the triplet is also not random, FaceNet [\cite{facenet}] introduces a negative data mining method which achieves faster and better convergence. The usual formulation of the triplet loss is  as follows:

% By pulling the representations of the same class together and pushing the representations of different far apart, triplet

% Triplet loss achieves the state-of-the-art results in metric learning and it is superior in learning large margin nearest neighbor embedding [\cite{LMNN}]. The representation is denoted by $h(x) \in \mathbb{R}^d$, the triplet loss is to want to ensure the representations of same class to be similar and the representations of different class to be dissimilar.  We call the pairing of the same class to be the positive pair, and the pair of different class to be negative pair. We want:



% \begin{equation}
% D(x_i^+, x_j^+) + \alpha < D(x_i^+, x_k^-)
% \end{equation}

%  The learning objective is minimizing the triplet loss over all given triplets:
% \[
% \sum_{i}^N \mathcal{L}_{trip}(\x_i, \x^+_i, \x^-_i)
% \]
% $x^+$ denotes the element of the positive pair and $x^-$ denotes the negative sample.






% $$\mathcal{L}_{pull} = \sum_{i,j \in +}D(x_i^+, x_j^+)$$

% $$\mathcal{L}_{push} = -\sum_{i \in +, k \in -}D(x_i^+, x_k^-)$$


